A Unified Framework for Fair Spectral Clustering With Effective Graph Learning

We consider the problem of spectral clustering under group fairness constraints, where samples from each sensitive group are approximately proportionally represented in each cluster. Traditional fair spectral clustering (FSC) methods consist of two consecutive stages, i.e., performing fair spectral embedding on a given graph and conducting $k$means to obtain discrete cluster labels. However, in practice, the graph is usually unknown, and we need to construct the underlying graph from potentially noisy data, the quality of which inevitably affects subsequent fair clustering performance. Furthermore, performing FSC through separate steps breaks the connections among these steps, leading to suboptimal results. To this end, we first theoretically analyze the effect of the constructed graph on FSC. Motivated by the analysis, we propose a novel graph construction method with a node-adaptive graph filter to learn graphs from noisy data. Then, all independent stages of conventional FSC are integrated into a single objective function, forming an end-to-end framework that inputs raw data and outputs discrete cluster labels. An algorithm is developed to jointly and alternately update the variables in each stage. Finally, we conduct extensive experiments on synthetic, benchmark, and real data, which show that our model is superior to state-of-the-art fair clustering methods.

==> Theory/theory.tex <==
In this section, we theoretically analyze the effect of the learned graph on the performance of FSC and the effect of fair spectral embedding on graph estimation.




\subsection{Question 1}
We utilize the smoothness-based GL model to learn similarity graphs underlying the observations for subsequent fair spectral embedding. Therefore, the quality of the learned graph inevitably affects the performance of FSC. The first question of concern is, \textit{given a graph learned by our model, what effect does this graph have on the final fair clustering results}? We assume that there are two or more meaningful ground-truth clusterings of the observed data, and only one of them is fair. As stated in \cite{kleindessner2019guarantees}, if there is only one meaningful clustering and this clustering is fair, then any existing clustering methods can recover the only fair clustering. To this end, we generate a random graph via the method in \cite{kleindessner2019guarantees}, which is a variant of the stochastic block model \cite{holland1983stochastic}. Here, we refer to the method as vSBM. Specifically, we assume $\mathcal{V}$ comprises $S$ sensitive groups and is partitioned into $K$ clusters such that $|\mathcal{D}_s \cap \mathcal{C}_k|/|\mathcal{C}_k| = \zeta_s, s\in [S], k\in[K]$, for $\zeta_s\in(0,1)$ with $\sum_{s=1}^S \zeta_s = 1$. In this way, we have the ground-truth fair clustering. Based on the clusters and sensitive groups, we construct a random graph by connecting two vertices $i,j$ with a certain probability $\mathrm{Pr}(i,j)$ that only depends on the clusters and sensitive groups of $i$ and $j$. For $i<j$, we let     
\begin{shrinkfix}
    \begin{align} 
    \mathrm{Pr}(i,j) =
\begin{cases}
a, & \pi_C(i) =  \pi_C(j), \; \pi_S(i) =  \pi_S(j)\\
b, & \pi_C(i) \neq  \pi_C(j),  \; \pi_S(i) =  \pi_S(j)\\
c, &  \pi_C(i) =  \pi_C(j),  \; \pi_S(i) \neq  \pi_S(j) \\
d, &  \pi_C(i) \neq  \pi_C(j),  \; \pi_S(i) \neq  \pi_S(j),
\end{cases}
    \label{eq-exper-1}
    \end{align}
\end{shrinkfix}
where $\pi_C: [D]\to [K]$ and $\pi_S: [D]\to [S]$ are two functions that assign a node $i\in\mathcal{V}$ to one of the clusters and groups. After obtaining connections among nodes, we can assign each edge a random weight. Next, we make the following assumptions.
\begin{assumption}
    Suppose $\widehat{\mathbf{U}}$ is the estimated continuous cluster indicator matrix, then for a given constant $\epsilon>0$, the $\widehat{\mathbf{Q}}$ and $\widehat{\mathbf{R}}$ estimated by spectral rotation of our model satisfies
\begin{shrinkfix}
    \begin{align} 
        \lVert \widehat{\mathbf{Q}} -  \widehat{\mathbf{U}}\widehat{\mathbf{R}}\rVert_{\mathrm{F}}^2 \leq (1+\epsilon) \underset{\mathbf{Q}\in\mathcal{I}, \mathbf{R}^{\top}\mathbf{R} = \mathbf{I}}{\min}\lVert {\mathbf{Q}} -  \widehat{\mathbf{U}}{\mathbf{R}}\rVert_{\mathrm{F}}^2.
    \label{eq-theo-res2-1}
    \end{align}
\end{shrinkfix}    
    \label{assump-1}
\end{assumption}
\begin{assumption}
The ground-truth clustering and sensitive partitions of $\mathcal{V}$ satisfies
\begin{shrinkfix}
    \begin{align} 
    |\mathcal{D}_s| = \frac{D}{S}, \; |\mathcal{C}_k| = \frac{D}{K}, \;\frac{|\mathcal{D}_s\cap\mathcal{C}_k|}{|\mathcal{C}_k|} = \frac{1}{S}.
    \label{eq-theo-res2-2}
    \end{align}
\end{shrinkfix}   
    \label{assump-2}
\end{assumption}
Assumption \ref{assump-1} is similar to the assumption of $(1+\epsilon)-$approximation of Kmeans \cite{lei2015consistency}, which provides the estimation error bound of spectral rotation in our model. Assumption \ref{assump-2} is the same as that of \cite{kleindessner2019guarantees}, which is made for ease of analysis. The conditions under which Assumption \ref{assump-2} is satisfied are discussed in \cite{kleindessner2019guarantees}. Based on the two assumptions, the clustering error of our model is provided as follows.


 
\begin{proposition}  
Under Assumptions \ref{assump-1}-\ref{assump-2}, let $\mathbf{L}^*$ be the ground-truth expected Laplacian matrix of the graph generated from the vSBM with probability $a>b>c>d$. Suppose $\widehat{\pi}_C(i)$ is the assigned cluster label of node $i$ output by Algorithm \ref{alg:1}, and define $\mathcal{M}_k:= \left\{i\in\mathcal{C}_k:\widehat{\pi}_C(i) \neq k  \right\}$ as the set of misclassified vertices of clutser $k$.  Then, the clustering returned by Algorithm \ref{alg:1} misclassifies at most
 \begin{shrinkfix}
    \begin{align} 
    \sum_{k=1}^K |\mathcal{M}_k|  \leq
\frac{256(4+2\epsilon)K^2}{D(c-d)^2}\lVert \mathbf{Z}^{\top}\mathbf{L}^*\mathbf{Z} - \mathbf{Z}^{\top}\widehat{\mathbf{L}}\mathbf{Z} 
    \rVert_{\mathrm{F}}^2,
    \label{eq-theo-res2-3}
    \end{align}
    \end{shrinkfix}  
where $\widehat{\mathbf{L}}$ is the estimated Laplacian matrix.
\label{theo-clustering performance}
\end{proposition}
\begin{proof}
The proof is inspired by \cite{kleindessner2019guarantees}. The main difference is that we use spectral rotation instead of Kmeans to obtain discrete clustering labels. Besides, Algorithm \ref{alg:1} is based on a graph learned from the observed data, while \cite{kleindessner2019guarantees} uses a graph that is regarded as a direct observation of the vSBM. See Appendix \ref{appendix2} for more details.
    \label{proof-theo-clustering performance}
\end{proof}

According to \cite{kleindessner2019guarantees}, the meaning of `` misclassify at most $D_{m}$ many vertices'' is that there exists a permutation of cluster indices such that the clustering results returned by our algorithm up to this permutation successfully predict all cluster labels but $D_{m}$ many vertices. Note that the clustering error bound depends on $K$ and $D$. It also depends on the approximation accuracy $\epsilon$ of spectral rotation. The term $\lVert \mathbf{Z}^{\top}\mathbf{L}^*\mathbf{Z} - \mathbf{Z}^{\top}\widehat{\mathbf{L}}\mathbf{Z} 
\rVert_{\mathrm{F}}^2$ indicates that a well-recovered graph $\widehat{\mathbf{L}}$, which is close to $\mathbf{L}^*$, brings a small misclassification error bound. Furthermore, the fair constraint affects clustering error bound via $\mathbf{Z}$. In the case that the graph estimation error $\lVert \mathbf{Z}^{\top}\mathbf{L}^*\mathbf{Z} - \mathbf{Z}^{\top}\widehat{\mathbf{L}}\mathbf{Z} 
\rVert_{\mathrm{F}}^2$ does not increase quadratically as $D$,  the fraction of misclassified vertices, which is equivalent to dividing the error bound of \eqref{eq-theo-res2-3} by $D$, will decay to zero as $D$ increases to infinity. Proposition \ref{theo-clustering performance} illustrates the importance of learning an accurate graph, and our model has the potential to learn an optimal graph for clustering, indicating better clustering performance. 











\subsection{Question 2}


Our model jointly learns graphs and performs fair spectral embedding, meaning that fair spectral embedding inevitably affects the learned graphs. Therefore, the second question we care about is that \textit{given the estimated fair spectral embedding $\widehat{\mathbf{U}}$, what is the effect of $\widehat{\mathbf{U}}$ on the learned graphs}? To this end, we calculated the upper bound of estimation error between ${\mathbf{L}}^*$ and $\widehat{\mathbf{L}}$ to illustrate the effect of fair spectral embedding on the learned graph. To simplify the calculation, it is not difficult to verify from \eqref{eq-prelim-2}  that the number of free variables of $\mathbf{L}$ is $D_f:= \frac{D\times(D-1)}{2}$, i.e., the number of upper triangle variables of $\mathbf{L}$. Therefore, we let $\mathbf{w}\in \mathbb{R}^{D_f}$ be the upper triangle variables of $\mathbf{L}$, and $Reg(\mathbf{L})$ is equivalent to $Reg_w(\mathbf{w}) = -\alpha\mathbf{1}^{\top}\log(\mathbf{S}\mathbf{w}) + 2\beta\lVert \mathbf{w}\rVert_2^2$, where $\mathbf{S}\in \mathbb{R}^{D\times D_f}$ is a linear operator satisfying $\mathbf{S}\mathbf{w} = \mathbf{W}\mathbf{1}$ \cite{kalofolias2016learn}. The following assumption is made based on the definition of $\mathbf{w}$.
\begin{assumption}
    The gradient of $Reg_w(\mathbf{w})$ is bounded, i,e, there exists a constant $C_R$ such that $\lVert \nabla_{\mathbf{w}}\, Reg_w(\mathbf{w})\rVert_{\mathrm{2}}\leq C_R$.
    \label{assump-r}
\end{assumption}
The assumption holds naturally when the underlying graph has no isolated nodes and finite edge weights. Then, we have the following Proposition. 

\begin{proposition}
    Under Assumption \ref{assump-r}, given $N$ observed data $\mathbf{X}\in\mathbb{R}^{D\times N}$,  suppose $\widehat{\mathbf{U}} = {\mathbf{Z}}\widehat{\mathbf{Y}}$ is the estimated fair spectral embedding. Then, the upper bound of estimation error between ${\mathbf{L}}^*$ and $\widehat{\mathbf{L}}$ is
    \begin{shrinkfix}
    \begin{align} 
&\lVert\widehat{\mathbf{L}} - {\mathbf{L}}^*\rVert_{\mathrm{F}} \notag\\
\leq &\underbrace{\frac{C_RC_D}{2\beta}}_{\mathcal{T}_1}+  \underbrace{\frac{C_D^2}{2\beta} \sqrt{C_X+  \frac{2\mu}{N}\mathrm{Tr}\left(\widehat{\mathbf{Y}}^{\top} \left(\mathbf{Z}^{\top}{\mathbf{X}}{\mathbf{X}}^{\top}{\mathbf{Z}}\right) \widehat{\mathbf{Y}}\right)  + K\mu^2}}_{\mathcal{T}_2}, 
    \label{eq-theo-graph-1}
    \end{align}
\end{shrinkfix}
where $C_D:= \sqrt{2}(\sqrt{(D-1)} + 1)$ and $C_X :=\frac{1}{N^2}\mathrm{Tr}\left(\mathbf{X}\mathbf{X}^{\top} {\mathbf{X}}{\mathbf{X}}^{\top}\right)$ are two constants determined by $\mathbf{X}$.
\label{theom-graph-estimation}
\end{proposition}
\begin{proof}
        See Appendix \ref{appendix1} for more details.
    \label{proof-theom-graph-estimation}
\end{proof}
Note that the proposition provides the upper bound (worst-case) on graph estimation error given data $\mathbf{X}$ and $\widehat{\mathbf{U}}$.  The bound consists of two terms $\mathcal{T}_1$ and $\mathcal{T}_2$, where $\mathcal{T}_1$ is determined by the regularizer $Reg_w(\mathbf{w})$, and the second term  $\mathcal{T}_2$ is determined by the observed data and the fair spectral embedding $\widehat{\mathbf{U}}$. Compared with independent graph construction without fair spectral embedding \cite{kalofolias2016learn}, our model will incur two additional terms related to $\widehat{\mathbf{U}}$ in $\mathcal{T}_2$, i.e., $\frac{2}{N}\mathrm{Tr}\left(\widehat{\mathbf{Y}}^{\top}\left(\mathbf{Z}^{\top}\mathbf{X}\mathbf{X}^{\top}{\mathbf{Z}}\right) \widehat{\mathbf{Y}}\right) +K$.  Specifically, $K$ is the predefined number of  clusters, and $\frac{2}{N}\mathrm{Tr}\left(\widehat{\mathbf{Y}}^{\top}\left(\mathbf{Z}^{\top}\mathbf{X}\mathbf{X}^{\top}{\mathbf{Z}}\right) \widehat{\mathbf{Y}}\right)$ is determined by the relationship between $\mathbf{X}$ and $\widehat{\mathbf{U}} = \mathbf{Z}\widehat{\mathbf{Y}}$. In a special case that $\widehat{\mathbf{Y}}$ contains the first $K$ eigenvectors of $\mathbf{Z}^{\top}\mathbf{X}\mathbf{X}^{\top}{\mathbf{Z}}$, the term  will reach the minimum
$\sum_{k=1}^K\mathrm{eig}_k(\mathbf{Z}^{\top}\mathbf{X}\mathbf{X}^{\top}{\mathbf{Z}})$  \cite{fan1949theorem}. Finally, the additional two terms induced by our model do not mean that our model is inferior to traditional GL models in graph inference since the error bound in \eqref{eq-theo-graph-1} is the possible maximum estimation error, not the real estimation error.


